Discovery of a Damped Ly-alpha System in a Low-z Galaxy Group: Possible Evidence for Gas Inflow and Nuclear Star Formation

We present a low-redshift (z=0.029) Damped Lyman-alpha (DLA) system in the spectrum of a background Quasi-Stellar Object (QSO). The DLA is associated with an interacting galaxy pair within a galaxy group. We detected weak Lyman-alpha emission centered at the absorption trough of the DLA. The emission was likely tracing the neutral HI reservoir around the galaxies in the interacting pair, which scattered the Lyman-alpha generated by star formation within those galaxies. We also found that the interacting pair is enveloped by a large HI cloud with $M(HI)=2\times 10^{10}M_{\odot}$. We discovered blueshifted 21cm HI emission, corresponding to M(HI)=$ 2\times10^{9}~M_{\odot}$, associated with J151225.15+012950.4 - one of the galaxies in the interacting pair. The blueshifted HI was tracing gas flowing into the galaxy from behind and towards us. Gas at similar blueshifted velocities was seen in the QSO sightline thus suggesting the presence of a filamentary structure of the order of 100kpc feeding the galaxy. We estimated a mass inflow rate of $2 M_{\odot}~yr^{-1}$ into the galaxy, which matches the star formation rate estimated from H-alpha emission. It is likely that the inflow of enormous amounts of gas has triggered star formation in this galaxy. The sudden acquisition of cold gas may lead to a starburst in this galaxy like those commonly seen in simulations.

==> corrections.tex <==
toward
quasi-stellar object
low-redshift

Unfortunately, at very low-redshifts, there are only a handful of DLAs that have been identified
cold-gas
, where
SDSS-based
in the range of  (instead of ranging from)
SFRs for a range
bla, bla, bla bla, bla bla, and bla bla
first,
absorbers, as well as
Decl.
log 
Figure shows the SDSS image of the group, with  -> the comma
orders of magnitude
were star-forming, with specific -> the comma
star formation rates (sSFRs)  --> the "s" at the end
f galaxy A, it was left out of the sample, as the sight line -> the comma
data on the galaxies, which were   -->  data is plural
We obtained the ultraviolet spectrum 

{\it Hubble Space Telescope}
1157 $-$ 1472$\rm \AA$ --> 1157 to 1472$\rm \AA$
 further out  -->  farther out
 de-blended --> deblended
similar to discussed by  -> similar to the discussed by 
 coronagraph
 both the absorption and the emission --> the "the" needed
 Equivalent width and column density corresponds 3$\sigma$  --> "corresponds "
 line-spread
 rest frame
 curve-fitting
 were derived from \Lya alone, as we did  --> the comma
 \ion{Si}{2} $\lambda\lambda$ 1190, 1193, 1260, and 1304;  --> double lambda
 low ionization 
 low ionization states, such as...
 saturated, thus
 of silicon
 best-fit 
 nondetection 
 absorption line
 of the DLA, as most
 were the dominant ones, as well as due
 As expected,
  two adjacent ionization states of silicon
 transitions, such as \ion{O}{1}, \ion{Si}{2}, and \ion{C}{2}, 
 cannot
 beam size
 4 and 2 hr, respectively. 
 signal-to-noise ratio
 lay close to one such extension; however, 
  C, respectively.
  Here we discuss
 the nature and location of the DLA were 
  similar velocities as the blueshifted-->  similar velocities to the blueshifted
 \HI-deficient
 environment, where 
 the low metallicity and the low ionization state
 red-band
 gray scale
 although of lower spatial resolution  --> add the "of"
 any sign of perturbation, suggesting
 low-velocity dispersion
 unusual in an undisturbed disk but are prevalent ---> no comma before but
 likely to exist since
  we estimate that the limiting \HI mass of such a galaxy would have to be no more than  --> that the
  an SFR surface density 
  an SFR of 
  X-ray-bright
  expected, as \Lya 
  an \Lya 
  either (1) 
  outflowing gas; instead, it was tracing
  \citep[see, e.g.][]{sembach03}
  accretion rate of gas to be  $\sim \rm 2 $
  metallicity to be the same as the DLA  -> "the"
  Lyman limit system (LLS )
  density of the LLS was in the range of
  east to west
  blueward
  cartoon describing two possible scenarios (inflow and outflow) that explain the possible 
  emission lines
  assuming a solar abundance ratio  --> the "a"
  we imaged the group in the \HI 21cm hyperfine transition   --> "the"
  Based on the proximity to the \HI --> Based on the proximity of the \HI
  H$\alpha$-producing
  was rejected due to the  ->> was rejected owing to the
  provide us with valuable --> the "with"  
  interaction-driven
  Single-dish
  dual-polarization
  expected; as the GBT
  using a method similar to the analysis by
  
  
  
 Fig Cap:  
 COS spectrum shows the \Lya absorption  --> COS spectrum showing the \Lya absorption
 gray 
 Middle: optically 
is shown in the lower left corner
LEFT: comparison
left-hand

















 
